IRIS: LLM-Assisted Static Analysis for Detecting Security Vulnerabilities

Software is prone to security vulnerabilities. Program analysis tools to detect them have limited effectiveness in practice due to their reliance on human labeled specifications. Large language models (or LLMs) have shown impressive code generation capabilities but they cannot do complex reasoning over code to detect such vulnerabilities especially since this task requires whole-repository analysis. We propose IRIS, a neuro-symbolic approach that systematically combines LLMs with static analysis to perform whole-repository reasoning for security vulnerability detection. Specifically, IRIS leverages LLMs to infer taint specifications and perform contextual analysis, alleviating needs for human specifications and inspection. For evaluation, we curate a new dataset, CWE-Bench-Java, comprising 120 manually validated security vulnerabilities in real-world Java projects. A state-of-the-art static analysis tool CodeQL detects only 27 of these vulnerabilities whereas IRIS with GPT-4 detects 55 (+28) and improves upon CodeQL's average false discovery rate by 5% points. Furthermore, IRIS identifies 4 previously unknown vulnerabilities which cannot be found by existing tools. IRIS is available publicly at https://github.com/iris-sast/iris.

==> background.tex <==
\section{Background}




==> discussion.tex <==
\section{Discussion and Future Work (0.33)}
\mypara{LLMs, including smaller ones, can produce high-quality taint specifications}
\Fix{talk about replacing codeql specs}

\mypara{Larger LLMs are better at context-based reasoning for filtering false alarms}

\mypara{Many vulnerabilities still remain hard to detect for static analysis}

\mypara{Deeper integration of static analysis with LLMs in necessary}


==> old-approach.tex <==
\section{\tool Overview (2.5)}

% \begin{figure}[!htb]
%     \includegraphics[width=\linewidth]{figures/pipeline.pdf}
%     \caption{An illustration of \tool's pipeline.}
%     \label{fig:pipeline}
% \end{figure}

\tool is a static analysis technique that detects vulnerabilities in Java
libraries. \tool is inherently neuro-symbolic: it combines the strengths of
static dataflow analysis and large language models to perform project-level
analysis to detect security vulnerabilities. We designed \tool to perform
vulnerability class (or CWE)-specific analysis. Because each vulnerability class
may differ in terms of where the malicious inputs come from (sources) or how the
tainted data is consumed (sinks), this approach allows us to customize our
approach for each class and perform a more focused analysis. Further, \tool's
architecture makes it easily extensible to any vulnerability class.

At a high level, \tool takes a Java project $P$, the
vulnerability class $C$ to detect, and a large language model $\texttt{LLM}$, as inputs.
\tool statically analyzes the project $P$, checks for vulnerabilities specific to $C$, and returns a set of potential security alerts $A$. 
Each alert is accompanied by a unique code path from a taint source to a taint sink that is vulnerable to $C$ (i.e., the path is unsanitized).

As illustrated in Fig.~\ref{fig:pipeline}, \tool has four main stages: 
First, \tool builds the given Java project and uses static analysis to extract all candidate APIs, including invoked external APIs and internal function parameters.
% external (or third-party) APIs used in the project. 
Second, \tool queries an LLM to label these APIs as sources or sinks that are specific to the given vulnerability class $C$. 
Third, \tool transforms the labelled sources and sinks into specifications that can be fed into a static analysis engine, such as CodeQL, and runs a \vulc-specific taint analysis query to detect vulnerabilities of that class in the project. 
This step generates a set of vulnerable code paths (or alerts) in the project. 
Finally, \tool triages the generated alerts by automatically filtering false positives, and presents them to the developer.

\Comment{
Algorithm~\ref{algo:main} describes the main algorithm of \tool. \Fix{we can
remove the algo if we have workflow diagram.}\mayur{I propose to remove the algorithm and use a workflow diagram.} We next describe the main
components of \tool.

% write an algorithm
\begin{algorithm}
    \caption{\tool Algorithm}
    \label{algo:main}
    \begin{algorithmic}[1] 
        \State \textbf{Input:} Project $P$, Version $V$, Vulnerability Class $T$, LLM $M$
        \State \textbf{Output:} Alerts $A$
        \State $\textit{Sources}_C \gets \textit{GetCandidateSources}(P, V)$
        \State $\textit{Sinks}_C \gets \textit{GetCandidateSinks}(P, V)$
        \State $\textit{Sources}_L \gets \textit{LabelSources}(\textit{Sources}_C, M, T)$
        \State $\textit{Sinks}_L \gets \textit{LabelSinks}(\textit{Sinks}_C, M, T)$
        \State $A \gets \textit{TaintAnalysis}(P, V, T, \textit{Sources}_L, \textit{Sinks}_L)$
        \State $A \gets \textit{FilterFalsePositives}(A, M, T)$
        \State \textbf{return} $A$
    \end{algorithmic}
\end{algorithm}
}



\subsection{Problem Statement}
We formally define the static taint analysis problem for vulnerability detection. Given a project $P$ consisting of several files and methods, taint analysis extracts an inter-procedural data flow graph $\mathbb{G} = (\mathbb{V}, \mathbb{E})$, where $\mathbb{V}$ is the set of nodes representing program expressions and statements, and $\mathbb{E} \subseteq \mathbb{V} \times \mathbb{V}$ is the set of edges representing data or control flow edges between the nodes. A vulnerability detection task comes with two sets $\boldsymbol{V}^C_\textit{source} \subseteq \mathbb{V}$, $\boldsymbol{V}^C_\textit{sink} \subseteq \mathbb{V}$ that denote source nodes where tainted data may originate and sink nodes where a security vulnerability can occur if tainted data reaches it, respectively. Naturally, different classes $C$ of vulnerabilities (or CWEs) have different source and sink specifications. Additionally, there can be sanitizer specifications, $\boldsymbol{V}^C_\textit{sanitizer} \in \mathbb{V}$, that block the flow of tainted data (such as escaping special characters in strings). 

The goal of taint analysis is to find pairs of sources and sinks, ($V_s \in \boldsymbol{V}^C_\textit{source}, V_t \in \boldsymbol{V}^C_\textit{sinks}$), such that there is an \emph{unsanitized} path from the source to the sink. More formally,
$\textit{Unsanitized\_Paths}(V_s, V_t) = \exists\text{ }\textit{Path}(V_s, V_t) \text{ s.t. } \forall V_n \in \textit{Path}(V_s, V_t), V_n \notin \boldsymbol{V}^C_\textit{sanitizer}$. Here, $\textit{Path}(V_1, V_k)$ denotes a sequence of nodes $(V_1, V_2, \ldots, V_k)$, such that $V_i \in \mathbb{V}$ and $ \forall i \in 1 \textit{ to } k-1: (v_i, v_{i+1}) \in \mathbb{E}$.

A project may use various third-party APIs whose specifications (i.e., source or sink) may be unknown -- reducing the effectiveness of taint analysis. 
In addition, internal APIs might accept untrusted input from downstream libraries as well.
Hence, our goal is to automatically infer specifications for such APIs. 
We define a specification $S^C$ as a 3-tuple $\langle T, F, R \rangle$, where $T \in \{\textit{ReturnValue}, \textit{Argument}, \textit{Parameter}, \ldots\ \}$ is the type of node to match in $\mathbb{G}$, $F$ is an N-tuple of strings describing the package, class, method name, signature, and argument/parameter position (if applicable) of an API, and $R \in \{\textit{Source}, \textit{Sink}, \textit{Sanitizer}\}$ is the role of the API. 
For example, the specification $\langle \textit{Argument}, (\texttt{java.lang}, \texttt{Runtime}, \texttt{exec}, (\texttt{String[]}), 0), \textit{Sink} \rangle$ denotes that the first argument of \texttt{exec} method of \texttt{Runtime} class is a sink for a vulnerability class (OS command injection). A static analysis tool
%, $M: \boldsymbol{S}^C_R \rightarrow \boldsymbol{V}^C_R$
maps these specifications to sets of nodes $\boldsymbol{V}^C_\textit{source}$ or $\boldsymbol{V}^C_\textit{sink}$ in $\mathbb{G}$. 

We develop an automated specification inference technique $\textit{LabelSpecs}(\boldsymbol{S}^{\#}, \texttt{LLM}, C, R) = \boldsymbol{S}_{R}^{C}$, where $\boldsymbol{S}^{\#}$ are candidate specifications for sources and sinks. In this work, we do not consider sanitizer specifications, because they typically do not vary for the vulnerability classes that we consider.
%
\Comment{Given a project, we consider various candidate specifications that involve external API calls and build specification inference methods for sources and sinks $L_\textit{source}: \boldsymbol{S}_\textit{source}^\textit{candidates} \mapsto \boldsymbol{S}_\textit{source}^{C}$ and $L_\textit{sink}: \boldsymbol{S}_\textit{sink}^\textit{candidates} \mapsto \boldsymbol{S}_\textit{sink}^{C}$, where $C$ is a vulnerability class. For sources, we consider the return values of third-party APIs, and for sinks, we consider the function arguments, as candidates.} 
%
As we show later in our evaluation, there can be up to \emph{tens of thousands} of such candidates per project with unknown specifications, making manual labeling impractical. We show how one can leverage LLMs to automatically infer such specifications. 

Further, even a few hundred taint specifications can produce thousands of $\textit{Unsanitized\_Paths}(V_s, V_t)$ that a developer needs to triage and many of such paths are false positives. In order to reduce the developer burden, we also develop an LLM-based filtering method, $\textit{FilterPath}(\textit{Path}, \mathbb{G}, \texttt{LLM}, C) = \texttt{True}|\texttt{False}$ that classifies a detected vulnerable path (\textit{Path}) in $\mathbb{G}$ as a true or false positive by leveraging context-based and natural language information.


%, such as function call sites, function arguments, and function formal parameters.


\subsection{Candidate Source/Sink Extraction}
\Comment{To perform taint analysis, we require \emph{taint specifications} -- APIs that
return potential sources of malicious user inputs (known as taint
\emph{sources}) and APIs that should not consume such malicious data without proper
sanitization (known as taint \emph{sinks}). Third-party libraries do
not come with such specifications, which makes taint analysis and consequently,
vulnerability detection challenging.}

To identify taint specifications $\boldsymbol{S}_\textit{source}^{C}$ and 
$\boldsymbol{S}_\textit{sink}^{C}$, 
we first extract $\boldsymbol{S}^{\#}$, third-party library APIs that are
invoked in the given Java project and are potential candidates 
to be taint sources or sinks. For this step, we develop a query using CodeQL's query language that
searches for calls to APIs not defined (hence external) in the given project.
For each invoked API, we extract metadata such as the method name, method
signature, class name and package name of the method.
\Comment{Listing~\ref{lst:extractapis} presents our CodeQL query that extracts
external APIs from a Java project.} \Comment{The extracted metadata is useful when
querying LLMs to label the APIs as potential sources or sinks.}

While extracting external APIs, we filter out commonly-used Java libraries that
are unlikely to contain any potential sources or sinks. Such libraries include
testing libraries like JUnit and Hamcrest or mocking libraries like Mockito.
%
While we filter out methods that are defined in the project, we specifically allow methods that are inherited from an external class or interface. 
An example is the \texttt{getResource} method of the generic class
\texttt{Class} in \texttt{java.lang} package, which takes a path as a string and accesses a file in the module. Many projects commonly inherit this class and use this method. 
If the input path is unchecked, it may lead to a Path-Traversal vulnerability if the path accesses resources outside the given module. Hence,
detecting such API usages is crucial.  

Taint sources are typically values returned by methods that obtain inputs
from external sources, such as response of an HTTP request or a command line
argument. 
Hence, we select external APIs that have a ``non-void'' return type as candidate sources. 
On the other hand, taint sinks are typically arguments to an external API. 
This involves \textit{explicit} arguments, such as the \texttt{command} argument passed to \texttt{Runtime.exec(String command)} method,
and \textit{implicit} \texttt{this} argument to non-static functions, such as the \texttt{file} variable in the function call \texttt{file.delete()}.
\Fix{add details about internal function params, we have it in figure 3}
% We consider arguments of such API as sink candidates.


% \begin{figure}[!htb]
%    \lstinputlisting[caption={Extract External APIs},style={codeqlstyle},label={lst:extractapis}]{code/fetch_apis.ql}
% \end{figure}


\subsection{Inferring Taint Specifications using LLMs}
We use LLMs to infer taint specifications, i.e., to label the external APIs as sources or sinks for each \vulc. 
The inferred specifications can then be fed into a static analysis engine, such as CodeQL, and used to perform taint analysis for the chosen \vulc. 
We do not infer sanitizer specifications and rely on CodeQL's existing sanitizers for each \vulc. 
This is mainly because sanitizers typically do not vary much for a given \vulc. 
Further, CodeQL does not track data flow through unknown functions, hence they act as sanitizers by default.

% We hypothesize that since LLMs are pre-trained on internet-scale data, they have knowledge about the behavior of widely used libraries and their APIs.
% Hence, it is natural to ask whether LLMs can be used to identify APIs that are
% relevant as sources or sinks for any \vulc. 
% \Comment{Currently, static analysis tools rely on manually identified specifications, which is labor-intensive and hard to scale, especially given the rapid development and evolution of libraries. } 
% If successful, LLMs can alleviate manual effort, and drastically
% improve the effectiveness of static analysis tools. 

\Comment{
There are a few key challenges in using LLMs for specification inference: First,
LLMs require natural language descriptions of a task (prompts) and have a
limited context window. Given that there may be thousands of external APIs in
the project, how do we design a prompt that can succinctly describe the
specification inference problem, describe the \vulc of interest, and allow LLMs
to effectively label them as sources or sinks? Further, even if some LLMs allow
large contexts (e.g., more than 100,000 tokens), LLMs have been shown to be
particularly unreliable when dealing with information in the middle of long
contexts~\cite{liu2024lost}. Hence, it is impractical to query LLMs using a
single large prompt. \Comment{Second, due to their probabilistic nature LLMs may
sometimes mislabel specifications, reducing their effectiveness. We discuss
how we tackle these challenges through carefully designing prompts and
additional context-based filtering strategies.}
}
% \Comment{Hence, it is important to estimate the
% \emph{confidence} of LLMs for each specification they infer. Such a confidence
% measure can help us in minimizing false positive security alerts returned by the
% static analysis engine.}

% \mypara{LLM Prompt Design for Specification Inference}
Fig.~\ref{fig:motivating-llm-label} shows partial user prompts for inferring source and sink specification from external API and internal function parameter candidates.
The full system- and user-prompts are shown in Listings~\ref{lst:prompt-api} and~\ref{lst:prompt-func-param} in the appendix.
\todo{Ziyang: I'm here}

\mypara{External API Specifications}
External APIs can be treated 

\mypara{Internal Function Parameter Specifications}


\todo{Update prompts in appendix}
For infering source and sink specifications, we design a custom system prompt that asks the LLM to assume the role of a security expert and describe the specification inference task. 
We describe what are taint sources or sinks and instruct the LLM to return the results only in a fixed format: a json list, which makes it easier to parse the results. 
In the user prompt, we describe the vulnerability class of interest in the \texttt{[CWE\_DESCRIPTION]} field and the cwe id in the \texttt{[CWE\_ID]} field. 
The rest of the prompt then lists several methods, one per line, with their package, class, method, and signature. Because, sinks are typically function arguments, we instruct the LLM to return the argument indices that are likely to be sinks. 
Listings~\ref{lst:promptsource} and~\ref{lst:promptsink}, in appendix, 
present the prompts that we designed for inferring specifications for sources and sinks
respectively.

\Comment{
In our initial experiments, we found that specifying the signature of
methods produces more consistent results and enables LLMs to accurately infer
the type and purpose of each argument -- which is especially important for sink
inference and handling overloaded methods. Because there may be thousands of
external API calls, we break down the LLM calls into smaller batches. We found
that a batch size of 50 achieves a good balance between context window limits
and result consistency. 

Further, we observed that GPT-4 was very restrictive in its results and only
labeled very few APIs. On closer inspection with an additional explanation
field, we found that GPT-4 often responded that the nature of the API is
context-dependent and hence it cannot be certain of its nature. For instance,
for an API to be a sink, the input data must be malicious. Hence, we append the
user prompt for sinks to assume that the inputs to presented API can be
\emph{potentially malicious}. For sources, we added an additional instruction
specifying that the method may also be invoked on objects that contain
unsanitized user inputs. A common source of this kind is the
\texttt{getRequestURI} method of the \texttt{HttpServletRequest} class that
returns URL components from the protocol name to the query string from a servlet
request object built from a user request. We observed that these instructions
remarkably improved the quality of the inferred specifications.
}


\subsection{Vulnerability Detection}
Once we obtain all the source and sink specifications from the LLM, the next
step is to combine it with a static analysis engine to detect vulnerable paths, i.e., 
$\textit{Unsanitized\_Paths}(V_s, V_t)$, in a given project.
In this work, we use CodeQL~\cite{codeql-web} for this step. CodeQL represents
programs as data flow graphs and provides a query language, akin to Datalog \cite{smaragdakis2010using},
to analyze such graphs. Many security vulnerabilities and bugs can be modeled using \emph{queries}
written in CodeQL and can be executed against data flow graphs extracted from
such programs. \Comment{CodeQL supports language-specific database schema and data
structures for languages such as C/C++, Java, Python, and JavaScript.} Given a data flow graph $\mathbb{G}^P$ of a project $P$, CWE-specific
source and sink specifications, and a query for a given vulnerability class $C$, CodeQL returns a set of 
unsanitized paths in the program.
Formally, 
\begin{equation}
\textit{CodeQL}(\mathbb{G}^{P}, \boldsymbol{S}_\textit{source}^{C}, \boldsymbol{S}_\textit{sink}^C, \textit{Query}^C) \rightarrow \{\textit{Path}_1, \ldots, \textit{Path}_k\}
\end{equation}
\Comment{CodeQL provides specific queries for detecting many common classes of vulnerabilities.}
CodeQL itself contains numerous specifications of third-party
APIs for each \vulc. However, as we show later in our evaluation, despite having
such specialized queries and extensive specifications, CodeQL fails to detect a
majority of vulnerabilities in real-world projects. For our analysis, we write a
specialized CodeQL query for each vulnerability that uses our mined
specifications instead of those provided by CodeQL. 
Our query for Path Traversal vulnerability (CWE 22) is shown in Listing~\ref{lst:cwe22} in the appendix.
We develop similar queries for each CWE that we evaluate.

\subsection{Triaging of Alerts via Contextual Analysis}

\begin{figure}[!htb]
    \includegraphics[width=\linewidth]{figures/contextual-analysis-prompt.pdf}
    \caption{
      LLM user prompt and response for contextual analysis of data-flow paths. 
      We modify the snippets and left out the system prompt for clearer presentation.
    }
    \label{fig:contextual-analysis-prompt}
    % \lstinputlisting[style=mypromptstyle,caption={LLM Prompt for Context-based Filtering of False Alarms},label={lst:filterprompt}]{code/filteringprompt.txt}
\end{figure}

Inferring taint specifications only solves part of the challenge. 
% since static analysis may still produce alerts that are false positives. 
We observe that while LLMs help uncover many new API specifications, sometimes they detect specifications that are not relevant to the \vulc being considered, resulting in too many predicted sources or sinks and consequently many spurious alerts as a result. 
% While one might consider tuning the LLMs or its prompts to improve the precision of specifications, this can lead to loss of recall, which cannot be otherwise recoverable. 
% Instead, we propose a filtering technique, namely \textit{Contextual Analysis}, that uses LLMs to reduce false alarms and further improve the precision of static analysis results. 
Our insight here is that providing sufficient relevant contextual information of a potentially vulnerable code path and targeting a specific \vulc allows LLMs to better reason about the code behavior.
Therefore, we propose \textit{Contextual Analysis} which classifies whether a produce path $\textit{Path}_i$ is likely a true positive or not.
% The goal is to generate whether a produced path $\textit{Path}_i$ is likely a true positive or not.

An example prompt for contextual analysis is illustrated in Fig.~\ref{fig:contextual-analysis-prompt}.
The prompt includes CWE information and code snippets for nodes along the path, with an emphasis on the source and sink.
Specifically, we include $\pm 5$ lines surrounding the exact source and sink location, as well as the enclosing function and class.
The exact line of source and sink is marked with a comment.
For the intermediate steps, we include the file names and the line of code.
When the path is too long, we keep only a subset of nodes to limit the size of the prompt.
As such, we provide the full context for the potential vulnerability to be thoroughly analyzed.

\Comment{
We expect the LLMs to produce JSON as the response, which includes the final verdict as well as an explanation to the verdict.
The format of the JSON suggests LLM to generate the explanation prior to the final verdict, since giving the judgement after the reasoning process is known to produce better results \todo{Cite Chain-of-thought}.
In addition, if the verdict is false, we ask the LLM to mark whether source or sink is a false positive.
This extra information helps to prune other paths so that we can save on the number of calls to the LLM.}

\Comment{Further, we also develop a User Interface (UX) that
allows developers to quickly triage through the alerts.}

%\subsubsection{Context-based Filtering of False Alarms} 

\Comment{
Distinguishing between a true
and false positive result requires understanding the context in which a source
or sink is used. Formally specifying such contextual rules is challenging.
Rather, we leverage LLMs to tackle this task. Our insight here is that providing
sufficient relevant contextual information of a potentially vulnerable code path
and targeting a specific \vulc allows LLMs to better reason about the code
behavior. Listing~\ref{lst:filterprompt} presents our custom LLM prompt template
that we developed for filtering static analysis alarms. We describe how we
populate this template.

CodeQL typically provides a code path starting from a source to a sink with
every security alert. For each such code path, we construct a prompt that
encodes the code path in a summary form. For the source and sink, we extract the
enclosing method and class, and few lines of code before and after the line
containing the source/sink, and include in the prompt. In particular, we replace
\texttt{[SOURCE\_STR]} with the source method and \texttt{[SOURCE\_CODE\_CONTEXT]}
with contextual information of the source. Similarly, we replace the
\texttt{[SINK\_STR]} and \texttt{[SINK\_CODE\_CONTEXT]} placeholder with sink
information. We also include the intermediate nodes in the code path in the
\texttt{[INTERMEDIATE\_STEPS]} block. For each intermediate node at step I, we
include the textual representation of the node in the following format:
\texttt{Step <I> [<FILE>:<FUNCTION>, <NODE\_STRING>]: <NODE\_FULL\_LINE>}, where
\texttt{NODE\_STRING} is the string representation of the node (such as the
method call expression), while the other terms have their usual meaning. Because
some code paths can be very long (up to 50 intermediate steps) and the LLM
context window is limited, we follow a simple heuristic to reduce the prompt
length. For paths longer than 10 intermediate steps, we only include alternate
nodes. In our experiments, we find that this helps limit the prompt length and
provide highly reliable results.
}


\Comment{
\subsubsection{User Interface for Triaging Alerts}
\Fix{we should remove this}
We developed a User Interface that makes it easier for developers to triage
through detected vulnerabilities. While CodeQL provides a plugin to view the
detected results and navigate the detected code paths, we find that it is
cumbersome for a developer to easily sift through many alerts. Further, there is
no way for developer to view similar alerts and eliminate or accept each group
easily. We developed a simple user interface that takes the output of \tool and
populates a Web UI with relevant information about each detected vulnerability.

Figure~\ref{fig:userinterface} shows a snapshot of the user interface for one
project and the details of the detected vulnerabilities. The UI provides
convenient options to mark each alert as a true positive or false positive (via
the \texttt{Is FP?} and \texttt{Is TP?} buttons). By default, the alerts are
grouped based on sink locations. The UI also provides a way to mark similar
alerts, i.e., alerts that share the same source or sinks, as true or false
positives. Developers can also quickly view the source code for each
intermediate node via a pop-up window using the URLs. Finally, the UI provides a
way to download the filtered alerts as a json file for further analysis. We
found that the UI was quite useful for our own analysis and understanding of the
vulnerabilities detected by \tool.

\begin{figure}[!htb]
    \centering
    \frame{\includegraphics[width=1.0\textwidth]{figures/ui.png}}
    \caption{User Interface for Triaging Alerts}
    \label{fig:userinterface}
\end{figure}
}


\subsection{Evaluation Metrics}
\Comment{
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=\linewidth]{figures/metrics.pdf}
  \end{center}
  \caption{
    A visualization of our metrics used for vulnerability detection, where the snippets are adapted from Zip4j v2.11.5-2, with slight changes for clearer presentation.
    While both sinks are potential causes of path-traversal (CWE-22), only the dataflow path on the right passes through the fixed sanitizer function.
    Therefore, we consider only the path on the right as a vulnerability.
  }
  \label{fig:metrics-visualization}
  % \mayur{this figure does not seem to be referenced anywhere in the text?}
\end{figure}
}
We evaluate the performance of \tool using two key metrics: 1) Recall: How many vulnerabilities can \tool detect successfully? and 2) Precision: Out of the vulnerabilities reported by \tool, how many are true vulnerabilities?
% We use the fix commit for each vulnerability to extract the file and methods locations that contain the fix.
% For each detected vulnerability, \tool reports code paths from a taint source to the taint sink. 
For evaluation, we assume that the label for a project $P$ is provided as a set of crucial program points $\mathbf{V}_{\text{fix}} = \{V_1, \dots, V_n\}$ where the vulnerable paths should pass through.
In practice, these are typically the patched methods that can be collected from each vulnerability report.
\Comment{As illustrated in Fig.~\ref{fig:metrics-visualization},} If at least one detected vulnerable path passes through a fixed location for the given vulnerability, then we consider the vulnerability detected.
Formally, it is defined as:
\begin{equation}
\textit{Recall}(\{\textit{Path}_i\}_{i=1}^k) 
= 
\mathbbm{1}_{|\{i |  \textit{Path}_i \cap \mathbf{V}_{\text{fix}} \neq \emptyset \}| > 0}
\end{equation}
In contrast to recall, computing the precision of the results is more challenging.
For instance, even if a detected code path does not intersect with a fixed file or method, it may actually point to a true vulnerability (e.g., a different CVE in the same version) in the project. Hence, we perform manual analysis needs to compute precision.



% We consider the
% following two ways to compute recall:
% \begin{itemize}
%     \item \textbf{Method-level Recall (\recallm):} If at least one detected code
%     path contains a fixed method.
%     \item \textbf{File-level Recall (\recallf):} If at least one detected code
%     path contains a fixed file.
% \end{itemize}
% \mayur{I would get rid of File-level Recall if it isn't used anywhere.}

% The Method-level Recall is expectedly stricter than the File-level Recall.
% However, in some cases, the fix for the vulnerability may only be at the class
% level (e.g., changing a static class variable). Hence, considering the
% File-level Recall is useful is such cases.



==> old-intro.tex <==
\section{Introduction (1.5 pages)}
Security vulnerabilities pose a major threat to the safety of software
applications and its users. Even after decades of advancements in programming
technologies and vulnerability detection tools, many widely used software
packages remain vulnerable to potential security issues. This is evident by the
ever increasing number of vulnerabilities (CVEs) reported each year. In 2023
alone, more than 29,000 CVEs were reported -- almost 4000 higher than  in 2022~\cite{cvedetails}. Hence, it is critical to rethink methods to automatically and proactively detect such vulnerabilities
before they can be exploited. 

\begin{figure}[h]
\includegraphics[width=\textwidth]{figures/banner.pdf}
\caption{
A high level overview of vulnerability detection process.
Given a full repository, we want to uncover whether it contains a certain type of weakness, as classified in Common Weakness Enumeration (CWE).
The end result is a dataflow path in the repository exposing the vulnerability, while indicating the unsanitized taint (source) and the direct cause (sink) of the weakness.
}
\label{fig:banner}
\vspace{-0.15in}
\end{figure}

Detecting security vulnerabilities in code is a challenging task. To
unmask a vulnerability, one needs to understand complex flow of program data
across multiple functions, classes, and modules. 
A promising and general technique called static taint analysis is widely used by developers and researchers to detect vulnerabilities.
Popular tools employing this technique, such as GitHub CodeQL~\cite{codeql}, Facebook Infer~\cite{fbinfer},
Checker Framework~\cite{checker}, and Snyk Code~\cite{synkio} provide different recipes (or analysis rules) to detect certain classes of vulnerabilities.
These tools, however, face several challenges that greatly limit their effectiveness and accessibility in practice.

%\mayur{Give more structure to below two paras by a bold header summarizing each challenge}

%\textbf{\textit{Missed Bugs due to Dependence on Taint Specifications.}}
\mypara{False negatives due to missing taint specifications of third-party library APIs}
First, static
taint analysis predominantly relies on \emph{specifications} of third-party
library APIs as sources, sinks, or sanitizers. 
%Intuitively, taint analysis works by marking certain program components that access user controlled data (known as taint \emph{source}), tracking the flow of such data throughout the program, and checking if such data flows into a sensitive API (known as taint \emph{sink}) without sanitization. For instance, if a server application accepts a cleverly masked command string through an http request (source) and executes the command without sanitization on its command line (sink), it can lead to a security exploit, also known as OS Command Injection.
In practice, developers and
analysis engineers have to manually craft such specifications based on their
domain knowledge and API documentation. \mk{give an idea of the large number of such specs, around ~10k for codeql, how many for Infer?} 
This is a laborious and
error-prone process that often leads to missing specifications and incomplete
analysis of vulnerabilities. Further, even if such specifications may exist for
many libraries, they need to be regularly updated to capture changes in newer
versions of such libraries and also cover new libraries that are developed.
As a result, obtaining such specifications is a never-ending and unscalable problem.

%\textbf{\textit{False Alarms from Need to Combine Logical and Intuitive Reasoning.}}
\mypara{False positives due to lack of precise context-sensitive and intuitive reasoning}
Second, it is well-known that static analysis often suffers from low precision,
i.e., it may often generate many false alarms~\cite{kang2022detecting,johnson2013don}. 
\mk{again, briefly give some numbers from CodeQL or Infer to communicate the sheer scale of the problem} 
Such imprecision may stem from
multiple sources. For instance, the source or sink specifications may be
spurious, or the analysis may over-approximate over branches in code or
potential program inputs. Further, even if the specifications are correct, the
context in which the detected source or sink is used may not lead to a
vulnerability. Hence, in reality, a developer may need to triage through numerous 
\mk{how many, whats the average false positive rate?}
(potentially false) security alerts, wasting developer time and effort.
Moreover, to triage each detected alert, a developer needs a combination of
different skills: domain expertise to understand the nature of the project being
analyzed and third-party library APIs, security expertise to assess the security
implications of a bug, and program analysis expertise to effectively use the
static analysis tool and distinguish between spurious and malicious alerts -- all of
which makes triaging alerts an extremely challenging and labor-intensive endeavor. 

\mypara{Limitations of existing data-driven approaches to improve static taint analysis} 
Many techniques have been proposed to address the challenges
of static taint analysis. For instance, Livshits~\etal proposed an automated
approach, MERLIN, to mine specifications from library
code~\cite{livshits2009merlin}. MERLIN models information flow paths in programs
using probabilistic constraints extracted from data propagation graphs and
solves these constraints using a factor graph to extract taint specifications. A
more recent work, Seldon~\cite{chibotaru2019scalable}, improved the scalability
of this approach by formulating the taint specification inference
problem as a linear optimization task. However, such approaches rely on analyzing
each third-party library to extract specifications, which is expensive and hard
to scale 
\mk{e.g. how many third-party libraries per project in the CWE-Bench-Java dataset?}. 
Researchers have also developed statistical analysis- and machine
learning-based techniques to mitigate false positive
alerts~\cite{jung2005taming,heckman2009model,ranking2014finding}. However,
recent studies~\cite{kang2022detecting} report that such approaches still have
limited effectiveness in practice. 
%\Fix{maybe some citations that target false warnings?}

Large Language Models (or LLMs) such as GPT-4 and Llama 3 have made impressive strides in code generation and summarization. LLMs have also been applied to code related tasks such as
program repair~\cite{xia2023automated}, code translation~\cite{pan2024lost},
test generation~\cite{lemieux2023codamosa}, and static
analysis~\cite{li2024enhancing}. Recent
studies~\cite{steenhoek2024comprehensive,khare2023understanding} evaluated LLMs'
effectiveness at detecting vulnerabilities at the method level and showed that
LLMs fail to do complex reasoning with code, especially because it depends on
the \emph{context} in which the method is used in the project. On the other
hand, recent benchmarks like SWE-Bench~\cite{jimenez2023swe} show that LLMs are
also poor at doing project-level reasoning. Hence, an intriguing question is
whether LLMs can be combined with static analysis to improve their reasoning
capabilities.

\subsection{Contributions of this work}
\mypara{Approach} In this work, we propose \textbf{\tool}, a novel neuro-symbolic approach for 
vulnerability detection that effectively combines the strengths of static analysis and LLMs and addresses the shortcomings of both techniques. Given
a project to analyze for a given \vulc (or CWE), \tool applies LLMs for detecting
CWE-specific taint specifications for third-party library APIs used in the
project. \tool then augments the inferred specifications with a static analysis tool,
such as CodeQL, and uses it to detect security vulnerabilities. Our intuition
here is because LLMs have seen numerous usages of such library APIs across
projects, they have an understanding of which APIs are relevant for different
\vulc{}es. 

Further, to address the imprecision problem of static analysis, we develop a contextual analysis technique 
with LLMs that drastically reduces the false positive alarms and minimizes the triaging effort for developers. Our key insight here
is that encoding the code-context and path-sensitive information in the LLM prompt
and focusing on a specific \vulc elicits more reliable reasoning from the LLM. 
%
Finally, our neuro-symbolic approach allows LLMs to do more precise whole-repository reasoning and minimizes the human effort involved in using static
analysis tools.

\mypara{Dataset} We curate a dataset of manually vetted and compilable Java projects, \textbf{\benchmark}, 
containing \totalvuls vulnerabilities (one per project) across four common vulnerability classes. The projects in the dataset are
complex, containing 300K lines of code on average, and 10 projects with more than a million lines of code, making it a challenging benchmark
for vulnerability detection.
%\todo{write about properties of this system that is better than LLM and static analysis}

\mypara{Results} We evaluate \tool on \benchmark 
using eight diverse open- and closed-source LLMs. Overall, \tool obtains the best results with GPT-4, detecting
\gptfourbugs vulnerabilities, which is \irismorebugsabs (\irismorebugsperc) more than CodeQL. Among open-source LLMs, DeepSeekCoder 7B, despite being much smaller than other LLMs performs the best, detecting \dscoderbugs vulnerabilities, followed by Llama 3 70B with \llamathreeseventybugs vulnerabilities.
Further, our \filtering technique reduces false positive alerts by \Fix{\irisfpreduction}\%.

    % Compared to CodeQL, \tool detects \irismorebugsabs (\irismorebugsperc) 
    % more vulnerabilities. Further, \tool's filtering strategy reduces false positive
    %  alarms by \Fix{\irisfpreduction}\% on average.

% In this paper, we make the following contributions:
% \begin{itemize}[leftmargin=*]
%     \item{\textbf{Approach:}} We propose a novel neuro-symbolic approach for
%     vulnerability detection that effectively combines static analysis and large
%     language models. We identify opportunities in static analysis where LLMs can
%     be most effective, thereby improving the overall performance and reducing
%     human effort in the process.
%     \item{\textbf{Context-based Filtering of False Alarms:}} We develop a
%     filtering technique that encodes potentially vulnerable program paths into LLM prompts
%     and reduces the number of false alerts in static analysis results.
%     \item{\textbf{Implementation:}} We implement our approach into a tool,
%     \tool. Currently, \tool supports detecting four vulnerability classes and is
%     extensible.
%     \item{\textbf{Dataset:}} We curate a dataset of manually vetted and
%     compilable Java projects, \benchmark, that contain \totalvuls vulnerabilities
%     across four different vulnerability classes. 
%     \item{\textbf{Experimental Evaluation:}} 
%     %\Fix{\tool also identifies new
%     % source and sink specifications that are missing in CodeQL. We sent ZZ Pull
%     % Request to CodeQL's developers to augment the inferred specifications to
%     % their suite.}
% \end{itemize}

Our dataset, tool, and results can be found at~\Fix{Link} and will be open-sourced upon publication.

==> problem.tex <==

\section{Problem Statement}
We formally define the static taint analysis problem for vulnerability detection. Given a project $P$ consisting of several files and methods, taint analysis extracts an inter-procedural data flow graph $\mathbb{G} = (\mathbb{V}, \mathbb{E})$, where $\mathbb{V}$ is the set of nodes representing program expressions and statements, and $\mathbb{E} \subseteq \mathbb{V} \times \mathbb{V}$ is the set of edges representing data or control flow edges between the nodes. A security specification comes with two sets $\boldsymbol{V}_\textit{source} \subseteq \mathbb{V}$, $\boldsymbol{V}_\textit{sinks} \subseteq \mathbb{V}$ that denote source nodes where tainted data may originate and sink nodes where a security vulnerability can occur if tainted data reaches it, respectively. Naturally, different classes of vulnerabilities (or CWEs) have different source and sink specifications. Additionally, there can be sanitizer specifications, $\boldsymbol{V}_\textit{sanitizers}$, that block the flow of tainted data (such as escaping special characters in strings). 

The goal of taint analysis is then to find pairs of sources and sinks, ($V_s \in \boldsymbol{V}_\textit{source}, V_t \in \boldsymbol{V}_\textit{sinks}$), in the project, such that there is at least one \emph{unsanitized} path from the source to the sink. More formally,
$\textit{Unsanitized\_Flows}(V_s, V_t) = \exists\text{ }\textit{Path}(V_s, V_t) \in G \text{ s.t. } \forall V_n \in \textit{Path}(V_s, V_t), V_n \notin \boldsymbol{V}_\textit{sanitizer}$.
%  V_s \in \boldsymbol{V}_\text{source}, V_t \in \boldsymbol{V}_\text{sinks},

% \mayur{In below two paras, give equal importance to the two challenges stated in the intro, and relate them to definition of UnsanitizedFlows, namely, 1) that labels for Vsource, Vsink, and Vsanitizer are typically missing and candidate sets are voluminous, and 2) that Path candidates are also voluminous (give scale of magnitude) and many are false alarms.}

A project may use various third-party APIs for which the specifications may be unknown -- reducing the effectiveness of taint analysis. Hence, our goal is to automatically infer source and sink specifications for such third-party APIs. We consider various candidate nodes in a given dataflow graph that use such APIs and develop specification inference methods for sources and sinks $L_\textit{source}: \boldsymbol{V}_\textit{source}^\textit{candidates} \mapsto \boldsymbol{V}_\textit{source}^{C}$ and $L_\textit{sink}: \boldsymbol{V}_\textit{sink}^\textit{candidates} \mapsto \boldsymbol{V}_\textit{sink}^{C}$, where $C$ is a vulnerability class. For sources, we consider the return values of third-party APIs, and for sinks, we consider the function arguments, as candidates. For this work, we do not consider sanitizer specifications, because they typically do not vary much for the vulnerability classes that we consider.

As we show later in our evaluation, there can be up to \emph{tens of thousands} of such candidates per project with unknown specifications, making manual labeling impractical. We show how one can leverage LLMs to automatically infer such specifications. Further, to resolve the false positive problems of static analysis we also develop an LLM-based filtering method that classifies a detected vulnerable path as a true or false positive by leveraging context-based and natural language information.


%, such as function call sites, function arguments, and function formal parameters.


==> tables/contextual-analysis.tex <==

\begin{table}[!tb]
\footnotesize
\centering
\caption{
Effectiveness of Contextual Analysis. 
We present the average number of reported vulnerable paths (\#Paths) and the number of detected vulnerabilities (\#Vuls)  after contextual analysis using LLMs across a subset of 40 projects.
The numbers in parentheses indicate the reduction in \#Paths (percentage) or detected vulnerabilities compared to before the contextual analysis.
\todo{Put this table into Ablation study; talk about the reduce of false positives}
}
\label{tab:contextual-analysis}
 \setlength{\tabcolsep}{3pt}
\begin{tabular}{c|rr|rr|rr|rr}
  \toprule
   \multirow{2}{*}{\textbf{CWE}}
   
   & \multicolumn{2}{c|}{\textbf{CodeQL}}    
     & \multicolumn{2}{c|}{\textbf{DeepSeekCoder 7B}}
       & \multicolumn{2}{c|}{\textbf{Llama 3 70B}} 
   & \multicolumn{2}{c}{\textbf{GPT-4}} \\
  \cmidrule{2-9}
         & \#Paths   & \#Vuls   & \#Paths (\%Red.)          & \#Vuls                     & \#Paths (\%Red.)           & \#Vuls                     & \#Paths (\%Red.)          & \#Vuls                     \\
  \midrule
  22           & 62       & 6        & 282 (\green{$\downarrow 59$\%})  & 7  (\green{$= 0$})  & 152 (\green{$\downarrow 46$\%}) & 7  (\green{$= 0$})  & 93 (\green{$\downarrow 70$\%})  & 10  (\green{$= 0$}) \\
 78           & 4        & 1        & 347 (\green{$\downarrow 55$\%})  & 4  (\red{$\downarrow 1$})  & 24 (\green{$\downarrow 42$\%})  & 2  (\green{$= 0$})  & 22 (\green{$\downarrow 95$\%})  & 3  (\red{$\downarrow 4$})  \\
 79           & 32       & 2        & 1002 (\green{$\downarrow 44$\%}) & 10  (\green{$= 0$}) & 406 (\green{$\downarrow 34$\%}) & 10  (\green{$= 0$}) & 350 (\green{$\downarrow 79$\%}) & 10  (\green{$= 0$}) \\
 94           & 0        & 0        & 1037 (\green{$\downarrow 50$\%}) & 7  (\green{$= 0$})  & 795 (\green{$\downarrow 34$\%}) & 7  (\green{$= 0$})  & 270 (\green{$\downarrow 82$\%}) & 6  (\red{$\downarrow 1$})  \\ \midrule
 \textbf{All} & 26       & 9        & 648 (\green{$\downarrow 50$\%})  & 28 (\red{$\downarrow 1$})   & 328 (\green{$\downarrow 36$\%}) & 26 (\green{$= 0$})   & 179 (\green{$\downarrow 81$\%}) & 29 (\red{$\downarrow 5$})   \\
      \bottomrule
   % \textbf{22}    & 172      & 22       & 89 (\green{$\downarrow 66$\%})  & 31  (\red{$\downarrow 3$}) & 288 (\green{$\downarrow 60$\%})  & 21  (\red{$\downarrow 1$}) & 158 (\green{$\downarrow 41$\%}) & 11 (\green{$=$})  \\
   % \textbf{78}    & 3        & 1        & 22 (\green{$\downarrow 87$\%})  & 3  (\red{$\downarrow 4$})  & 347 (\green{$\downarrow 39$\%})  & 5  (\red{$\downarrow 1$})  & 24 (\green{$\downarrow 74$\%})  & 2  (\green{$=$})  \\
   % \textbf{79}    & 31       & 4        & 350 (\green{$\downarrow 71$\%}) & 16  (\red{$\downarrow 1$}) & 1002 (\green{$\downarrow 33$\%}) & 10  (\green{$=$}) & 406 (\green{$\downarrow 34$\%}) & 10 (\green{$=$}) \\
   % \textbf{94}    & 1        & 0        & 270 (\green{$\downarrow 78$\%}) & 6  (\red{$\downarrow 5$})  & 1035 (\green{$\downarrow 48$\%}) & 9  (\green{$=$})  & 795 (\green{$\downarrow 34$\%}) & 7  (\green{$=$})  \\
   % \midrule
   % \textbf{All} & 87       & 27       & \textbf{181} (\green{$\downarrow 75$\%}) & \textbf{56} (\red{$\downarrow 13$}) & 658 (\green{$\downarrow 45$\%})  & 45 (\red{$\downarrow 2$})  & 334 (\green{$\downarrow 46$\%}) & 30 (\green{$=$})   \\

\end{tabular}
\vspace{-10px}

\end{table}

% \begin{table}[!htb]
% \footnotesize
% \centering
% \caption{Effectiveness of Posthoc Filtering. We present the average number of security alerts (\textbf{\posthocalerts}) and the number of detected vulnerabilities (\textbf{\dvuls})  after path-based filtering using LLMs. The numbers in parentheses indicate the reduction in alerts (percentage) or detected vulnerabilities after filtering.\Fix{VERSION 1}}
%  \setlength{\tabcolsep}{4pt}
% \begin{tabular}{l|rr|rr|rr|rr}\toprule
%   &   \multicolumn{2}{c|}{\textbf{CodeQL}} & \multicolumn{2}{c|}{\textbf{\llama{3 8b}}}   & \multicolumn{2}{c|}{\textbf{\gpt{3.5}}}  & \multicolumn{2}{c}{\textbf{\gpt{4}}}  \\ \cmidrule{2-9}
%       \textbf{CWE}  &   \textbf{\posthocalerts}  & \textbf{\dvuls} & \textbf{\posthocalerts} &  \textbf{\dvuls}   & \textbf{\posthocalerts} &  \textbf{\dvuls}   & \textbf{\posthocalerts} & \textbf{\dvuls}   \\ \midrule
 
%    22    & 172      & 22       & 409 (\green{$\downarrow 30$\%})  & 19  (\green{$\downarrow 0$}) & 33 (\green{$\downarrow 97$\%}) & 20  (\red{$\downarrow 7$}) & 45 (\green{$\downarrow 93$\%})  & 31  (\red{$\downarrow 3$}) \\
%  78    & 3        & 1        & 144 (\green{$\downarrow 43$\%})  & 2  (\red{$\downarrow 1$})  & 0 (\green{$\downarrow 100$\%}) & 0  (\red{$\downarrow 1$})  & 5 (\green{$\downarrow 94$\%})   & 3  (\red{$\downarrow 4$})  \\
%  79    & 31       & 4        & 825 (\green{$\downarrow 44$\%})  & 11  (\red{$\downarrow 2$}) & 5 (\green{$\downarrow 99$\%})  & 11  (\red{$\downarrow 4$}) & 140 (\green{$\downarrow 85$\%}) & 16  (\red{$\downarrow 1$}) \\
%  94    & 1        & 0        & 1564 (\green{$\downarrow 48$\%}) & 7  (\red{$\downarrow 5$})  & 6 (\green{$\downarrow 99$\%})  & 8  (\red{$\downarrow 2$})  & 83 (\green{$\downarrow 94$\%})  & 5  (\red{$\downarrow 6$})  \\ \midrule 
% \textbf{Avg/Total}    & 87       & 27       & 690 (\green{$\downarrow 38$\%})   & 39 (\red{$\downarrow 8$})   & 18 (\green{$\downarrow 98$\%})  & 39 (\red{$\downarrow 14$})  & 72 (\green{$\downarrow 91$\%})   & 55 (\red{$\downarrow 14$})  \\
% % 22 & 172   & 22     & 612/409   & 30\%      & 19/19    & 2107/33    & 97\%       & 27/20    & 760/45   & 93\%      & 34/31  \\
% %  78 & 3     & 1      & 282/144   & 43\%      & 3/2      & 73/0       & 100\%      & 1/0      & 529/5    & 94\%      & 7/3    \\
% %  79 & 31    & 4      & 1875/825  & 44\%      & 13/11    & 1446/5     & 99\%       & 15/11    & 2139/140 & 85\%      & 17/16  \\
% %  94 & 1     & 0      & 2663/1564 & 48\%      & 12/7     & 1146/6     & 99\%       & 10/8     & 1591/83  & 94\%      & 11/5   \\ \midrule
% %     & 87    & 27     & 1261/690  & 38\%      & 47/39    & 1548/18    & 98\%       & 53/39    & 1237/72  & 91\%      & 69/55  \\ 
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[!htb]
% \footnotesize
% \centering
% \caption{Effectiveness of Posthoc Filtering. We present the average number of security alerts (\textbf{\posthocalerts}) and the number of detected vulnerabilities (\textbf{\dvuls})  after path-based filtering using LLMs. The numbers in parentheses indicate the reduction in alerts (percentage) or detected vulnerabilities after filtering.\Fix{VERSION 2}}
%  \setlength{\tabcolsep}{3pt}
% \begin{tabular}{l|rr|rr|rr|rr}\toprule
%   &   \multicolumn{2}{c|}{\textbf{CodeQL}} & \multicolumn{2}{c|}{\textbf{\llama{3 8b}}}   & \multicolumn{2}{c|}{\textbf{\gpt{3.5}}}  & \multicolumn{2}{c}{\textbf{\gpt{4}}}  \\ \cmidrule{2-9}
%       \textbf{CWE}  &   \textbf{\posthocalerts}  & \textbf{\dvuls} & \textbf{\posthocalerts} &  \textbf{\dvuls}   & \textbf{\posthocalerts} &  \textbf{\dvuls}   & \textbf{\posthocalerts} & \textbf{\dvuls}   \\ \midrule
% 22 & 172   & 22     & 612/409   (\green{$\downarrow$ 30\%})      & 19/19    & 2107/33    (\green{$\downarrow$ 97\%})     & 27/20    & 760/45  (\green{$\downarrow$ 93\%})      & 34/31  \\
%  78 & 3     & 1      & 282/144   (\green{$\downarrow$ 43\%})     & 3/2      & 73/0       (\green{$\downarrow$ 100\%})      & 1/0      & 529/5    (\green{$\downarrow$ 94\%})      & 7/3    \\
%  79 & 31    & 4      & 1875/825  (\green{$\downarrow$ 44\%})    & 13/11    & 1446/5     (\green{$\downarrow$ 99\%})       & 15/11    & 2139/140 (\green{$\downarrow$ 85\%})      & 17/16  \\
%  94 & 1     & 0      & 2663/1564 (\green{$\downarrow$ 48\%})      & 12/7     & 1146/6     (\green{$\downarrow$ 99\%})      & 10/8     & 1591/83  (\green{$\downarrow$ 94\%})      & 11/5   \\ \midrule
%     & 87    & 27     & 1261/690  (\green{$\downarrow$ 38\%})      & 47/39    & 1548/18    (\green{$\downarrow$ 98\%} )      & 53/39    & 1237/72  (\green{$\downarrow$ 91\%})      & 69/55  \\ 
% \bottomrule
% \end{tabular}
% \end{table}


==> tables/cves-old.tex <==
\begin{table}[h!]
    \scriptsize
    \caption{
        An overview of a selection of evaluated CVEs from our dataset.
        To give a glimpse of scale, we show the Java line-of-code (LoC) with blank and comments excluded, along with number of external APIs invoked in the project.
        We additionally show individual comparisons between \tool and CodeQL.
        In the table, \alarm represents number of generated alarms, while \textbf{$\textit{R}_F$} and \textbf{$\textit{R}_M$} are shorthands for \textbf{\recallf} and \textbf{\recallm}, respectively.
    }
    \label{tab:vul-detect-detail}
    \begin{tabular}{c|ll|cc|ccc|ccc}
        \toprule
        \multirow{2}{*}{\textbf{CWE}} &
        \multirow{2}{*}{\textbf{CVE ID}} &
        \multirow{2}{*}{\textbf{Project}} &
        \multirow{2}{*}{\textbf{\#LoC}} &
        \multirow{2}{*}{\parbox{1.5cm}{\centering \textbf{\#External \\ APIs}}} &
        \multicolumn{3}{c|}{\textbf{\tool}}  &
        \multicolumn{3}{c}{\textbf{CodeQL}}   \\ \cline{6-11}
        &              &                & & & \textbf{\alarm} & \textbf{$\textit{R}_F$} & \textbf{$\textit{R}_M$} & \textbf{\alarm} & \textbf{$\textit{R}_F$} & \textbf{$\textit{R}_M$} \\ \midrule

        22        & CVE-2016-9177	& spark               & 10K    & 444   & 10     & \cmark   & \cmark   & 12   & \cmark    & \cmark   \\
        22        & CVE-2018-9159	& spark               & 10K    & 477   & 9      & \cmark   & \cmark   & 13   & \cmark    & \cmark   \\
        22        & CVE-2018-1047	& wildfly             & 480K   & 9618  & 91     & \cmark   & \xmark   & 29   & \xmark    & \xmark   \\
        22        & CVE-2018-12542	& vertx-web           & 34K    & 1210  & 10     & \cmark   & \cmark   & 0    & \xmark    & \xmark   \\
        22        & CVE-2018-17297	& hutool              & 136K   & 2542  & 54     & \cmark   & \cmark   & 22   & \cmark    & \cmark   \\
        22        & CVE-2016-10726	& DSpace              & 219K   & 4020  & 425	& \xmark   & \xmark   & 222  & \xmark    & \xmark   \\
        22        & CVE-2020-5410	& spring-cloud-config & 19K    & 1065  & 4      & \xmark   & \xmark   & 4    & \cmark    & \cmark   \\
        \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\
        \midrule

        78        & CVE-2022-25174	& workflow-cps-global-lib-plugin& 4K & 6819 & 1	& \cmark	& \xmark	& 0	& \xmark	& \xmark \\
        78        & CVE-2019-10392	& git-client-plugin& 17K & 1153 & 6	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        78        & CVE-2013-7285	& xstream& 44K & 1657 & 2	& \cmark	& \xmark	& 0	& \xmark	& \xmark \\
        78        & CVE-2022-20617	& docker-commons-plugin& 3K & 4403 & 4	& \xmark	& \xmark	& 1	& \xmark	& \xmark \\
        78        & CVE-2017-1000487	& plexus-utils& 23K & 2171	& 6	& \xmark	& \xmark	& 1	& \xmark	& \xmark \\
        78        & CVE-2022-33140	& nifi& 820K & 7270	& 1	& \xmark	& \xmark	& 20	& \cmark	& \cmark \\
        78        & CVE-2014-3576	& activemq& 315K & 2170	& 75	& \xmark	& \xmark	& 1	& \xmark	& \xmark \\
        \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\
        \midrule

        79        & CVE-2016-10006	& antisamy& 6K & 1296 & 29	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        79        & CVE-2019-10077	& jspwiki& 59K & 1379 & 375	& \cmark	& \cmark	& 21	& \xmark	& \xmark \\
        79        & CVE-2019-10219	& hibernate-validator& 88K & 1003 & 6	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        79        & CVE-2022-24891	& esapi-java-legacy& 36K & 2119 & 14	& \cmark	& \cmark	& 2	& \cmark	& \cmark \\
        79        & CVE-2018-1000129	& jolokia& 30K & 2075 & 42	& \cmark	& \cmark	& 1	& \cmark	& \cmark \\
        79        & CVE-2020-29204	& xxl-job& 9K & 585 & 36	& \xmark	& \xmark	& 0	& \xmark	& \xmark \\
        79        & CVE-2020-13973	& json-sanitizer& 2K & 6919	& 0	& \xmark	& \xmark	& 0	& \xmark	& \xmark \\
        \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\
        \midrule

        94        & CVE-2021-21345	& xstream& 53K & 14451	& 26	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        94        & CVE-2021-41269	& cron-utils & 13K & 259 & 4	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        94        & CVE-2020-17530	& struts& 162K & 4136 & 250	& \cmark	& \xmark	& 0	& \xmark	& \xmark \\
        94        & CVE-2022-22947	& spring-cloud-gateway& 26K& 1542 & 3	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        94        & CVE-2021-30180	& dubbo& 174K & 2955 & 27	& \cmark	& \cmark	& 0	& \xmark	& \xmark \\
        94        & CVE-2018-1260	& spring-security-oauth& 45K & 1554	& 21	& \xmark	& \xmark	& 0	& \xmark	& \xmark \\
        94        & CVE-2019-0222	& activemq& 408K& 7393 & 425	& \xmark	& \xmark	& 0	& \xmark	& \xmark \\
        \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots & \dots \\
        \midrule
    \end{tabular}
\end{table}

